Neural Configuration Distance Function for Continuum Robot Control

This paper presents a novel method for modeling the shape of a continuum robot as a Neural Configuration Euclidean Distance Function (N-CEDF). By learning separate distance fields for each link and combining them through the kinematics chain, the learned N-CEDF provides an accurate and computationally efficient representation of the robot's shape. The key advantage of a distance function representation of a continuum robot is that it enables efficient collision checking for motion planning in dynamic and cluttered environments, even with point-cloud observations. We integrate the N-CEDF into a Model Predictive Path Integral (MPPI) controller to generate safe trajectories for multi-segment continuum robots. The proposed approach is validated for continuum robots with various links in several simulated environments with static and dynamic obstacles.

==> tex/Background.tex <==
\section{Background}
\label{sec: background}
This section introduces our notation and offers a brief review of model predictive path integrals (MPPIs) and CBF-based safety filters.


\subsection{Notation}
\label{sec: notation}
The sets of real, non-negative real, and natural numbers are denoted by $\bbR$, $\bbR_{\geq 0}$, and $\bbN$, respectively. For $N \in \bbN$, we write $[N] := \{1,2, \dots N\}$. We use $\boldsymbol{0}$ and $\boldsymbol{1}$ to denote the vector with all entries equal to $0$ and $1$, respectively. For a scalar $x$, we define $(x)_+ := \max(x,0)$. We denote by $\bfI_n \in \bbR^{n \times n}$ the identity matrix. The interior and boundary of a set $\calC \subset \bbR^n$ are denoted by $\text{Int}(\calC)$ and $\partial \calC$. 
The gradient of a differentiable function $\map{V}{\bbR^n}{\bbR}$ is denoted by $\nabla V$, while its Lie derivative along a vector field $\map{\bff}{\bbR^n}{\bbR^n}$ is $\calL_{\bff} V  = \nabla V^\top \bff$. A continuous function $\alpha: [0,a)\rightarrow [0,\infty )$ is of class $\calK$ if it is strictly increasing and $\alpha(0) = 0$. A continuous function $\alpha: \bbR \rightarrow \mathbb{R}$ is of extended class $\calK_{\infty}$ if it is strictly increasing, $\alpha(0) = 0$, and $\lim_{r \rightarrow \infty} \alpha(r) = \infty$. 

\subsection{Model Predictive Path Integrals}

We consider a general, discrete non-linear system:
\begin{equation}
\label{eq: general_discrete_system}
    \bfx_{k+1} = \bff(\bfx_k, \bfu_k)
\end{equation}
%
where $\bfx_k \in \calX \subseteq \mathbb{R}^{n}$ is the  state, $\bfu_k \in \mathbb{R}^{m}$ is the control input
at time step $k$, and $\map{\bff}{\mathbb{R}^{n}}{\mathbb{R}^{n}}$ is locally Lipschitz.  

MPPI (model predictive path integrals) is an MPC scheme that works by sampling multiple control sequences (control rollouts) around a nominal sequence and propagating them through the system’s model. A new control sequence is evaluated as the weighted average of all rollouts (with weights computed according to some cost function) and is used to construct the
nominal control sequence for the next iteration. 


\subsection{CBF-based Safety Filter}

Consider a non-linear control-affine system,
%
\begin{equation}
\label{eq: dynamic}
    \dot{\bfx} = \bff(\bfx) +\bfg(\bfx) \bfu 
\end{equation}
%
where $\bfx \in \calX \subseteq \mathbb{R}^{n}$ is the  state, $\bfu \in \mathbb{R}^{m}$ is the control input, and $\map{\bff}{\mathbb{R}^{n}}{\mathbb{R}^{n}}$ and $\map{\bfg}{\mathbb{R}^{n}}{\mathbb{R}^{n \times m}}$ are locally Lipschitz continuous functions.  

% The notion of a control Lyapunov function (CLF)~\cite{Artstein1983StabilizationWR, SONTAG1989117} plays a key role in certifying the stabilizability of control-affine systems.

% \begin{definition}
% A continuously differentiable function $\map{V}{\bbR^n}{\bbR}$ is a \emph{control Lyapunov function} (CLF) on $\calX$ for system \eqref{eq: dynamic} if $V(\bfx)>0$, $\forall \bfx \in \calX \setminus \{\boldsymbol{0}\}$, $V(\boldsymbol{0}) = 0$, and
% %
% \begin{equation}\label{eq: clf}
%     \inf_{\bfu \in \bbR^m} \text{CLC}(\bfx,\bfu) \leq 0, \quad \forall \bfx \in \calX,
% \end{equation}
% %
% where $\text{CLC}(\bfx,\bfu) := \mathcal{L}_{\bff} V(\bfx) + \mathcal{L}_{\bfg} V(\bfx)\bfu + \alpha_V( V(\bfx))$
% is the \emph{control Lyapunov constraint} (CLC) defined for some class $\calK$ function $\alpha_V$.
% \end{definition}
%

To facilitate safe control synthesis, we consider a time-varying set $\calC(t)$ defined as the zero superlevel set of a continuously differentiable function $h: \calX \times \bbR_{\geq 0} \rightarrow \bbR$:
%
\begin{equation}
\label{eq: safe_set}  
    \calC(t) := \{\bfx \in \calX: h(\bfx, t) \geq 0 \}.
\end{equation}
%
Safety of the system \eqref{eq: dynamic} can then be ensured by keeping the state $\bfx$ within the safe set $\calC(t)$.

\begin{definition}
\label{def: tv_cbf}
A continuously differentiable function $h: \mathbb{R}^n \times \bbR_{\geq 0} \rightarrow {\mathbb{R}}$ is a \emph{time-varying control barrier function} (TV-CBF) on $\mathcal{X} \subseteq \mathbb{R}^n$ for \eqref{eq: dynamic} if there exists an extended class $\mathcal{K}_{\infty}$ function $\alpha_h$ with:
%
\begin{equation}\label{eq:tv_cbf}
    \sup_{\bfu\in \mathcal{U}} \text{CBC}(\bfx,\bfu, t) \geq 0, \quad \forall \; (\bfx,t) \in \calX \times \bbR_{\geq 0},
\end{equation}
where the \emph{control barrier constraint (CBC)} is:
\begin{align}
\label{eq:tvcbc_define}
    &\text{CBC}(\bfx,\bfu, t) := \dot{h}(\bfx, t) + \alpha_h(h(\bfx,t)) \\
    & = \mathcal{L}_{\bff} h(\bfx, t) + \mathcal{L}_{\bfg} h(\bfx, t)\bfu + \frac{\partial h(\bfx,t)}{\partial t} + \alpha_h(h(\bfx,t)). \notag
\end{align}
\end{definition}

Definition~\ref{def: tv_cbf} allows us to consider the set of control values $K_{\text{CBF}}(\bfx, t) := \left \{  \bfu \in \bbR^m: \text{CBC}(\bfx,\bfu, t) \geq 0 \right \}$ that render the set $\calC(t)$
forward invariant. 

\begin{definition}\label{def:tvfi}
%\longthmtitle{Time-Varying Forward Invariance}
Let $t_0$ be a fixed initial time. A time-varying set $\calC(t)$ is said to be \emph{forward invariant} under control law $\bfu : [t_0, \infty) \rightarrow \mathbb{R}^m$ if, for any initial state $\bfx_0 \in \calC(t_0)$, there exists a unique maximal solution $\bfx : [t_0, t_1) \rightarrow \mathbb{R}^n$ to the system dynamics in~\eqref{eq: dynamic} with $\bfx(t_0) = \bfx_0$, such that $\bfx(t) \in \calC(t)$ for all $t \in [t_0, t_1)$.
% where $t_1$ is the maximal time of existence of the solution.
\end{definition}
%
Suppose we are given a baseline feedback controller $\bfu = \bfk(\bfx)$ and we aim to ensure the safety and stability of the control-affine system \eqref{eq: dynamic}. By observing that the safety constraint \eqref{eq:tv_cbf} is affine in the control input $\bfu$, a quadratic program \cite{ames2016control} can be formulated to synthesize a safe controller:
%
\begin{equation}
\begin{aligned}
\label{eq: clf_cbf_qp}
    \bfu(\bfx, t) \in &\argmin_{\bfu \in \bbR^m } \| \bfu - \bfk(\bfx)\|^2  \\
    \mathrm{s.t.} \, \,  &\text{CBC}(\bfx,\bfu, t) \geq 0 .
\end{aligned}
\end{equation}






==> tex/CSDF_Verification.tex <==
\section{Formal Verification of the Learned Shape}
\label{sec: CSDF_Verify}

In this section, we verify the correctness of the learned shape of the continuum robot. 

\TODO{Can we verify the learned zero-levle set is accurate? Idea: for simplicity: can we verify the learned SDF?}

